Rigorous Q Factor Formulation and Characterization for Nonlinear Oscillators

In this paper, we discuss the definition of Q factor for nonlinear oscillators. While available definitions of Q are often limited to linear resonators or oscillators with specific topologies, our definition is applicable to any oscillator as a figure of merit for its amplitude stability. It can be formulated rigorously and computed numerically from oscillator equations. With this definition, we calculate and analyze the Q factors of several oscillators of different types. The results confirm that the proposed Q formulation is a useful addition to the characterization techniques for oscillators.

==> newcommands-colours.tex <==
% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings


==> newcommands-eg-ie-etc.tex <==
% eg, ie, etc, wrt, viz newcommands
\newcommand{\eg}{{\it e.g.\/}}
\newcommand{\ie}{{\it i.e.\/}}
\newcommand{\wrt}{{\it wrt}}
\newcommand{\viz}{{\it viz.\/}}
\newcommand{\vs}{{\it vs.\/}}
\newcommand{\aka}{{\it aka\/}}
\newcommand{\apriori}{{\it a priori}}
\newcommand{\etc}{\textit{etc.}}                                                
% etc defined so that there is only a single period after it if it is followed 
% by a period
% see: http://en.wikibooks.org/wiki/TeX/def                                      
% see: http://www.tug.org/pipermail/texhax/2004-July/002449.html                 
% see: http://en.wikibooks.org/wiki/TeX/if                                       
%\ifx \etc \undefined                                                             
%  %\def\myarg{#1}                                                                
%  %\def\myfullstop{.}                                                            
%  %\def\etc{#1}{\textit{etc} arg is ``\myarg'' \ifx\myarg\myfullstop\then.\else.#1\fi\/}
%  \def\etc#1{\textit{etc}\if#1..\else.#1\fi}                                     
%\fi                                                                              
%                        


==> newcommands-for-bibtex.tex <==
\newcommand{\BP}{({\textbf{Best Paper}})} % used in bibliography
\newcommand{\BPnom}{({\textbf{Best Paper Nomination}})} % used in bibliography
\newcommand{\IP}{({\textbf{Invited}})} % used in bibliography
\newcommand{\presenter}[1]{#1} % used in bibliography
\newcommand{\putDOI}[1]{#1}
%\newcommand{\putDOI}[1]{}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}


==> newcommands-highlight-ignore.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands for ignoring, commenting, annotating, highlighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\newcommand{\jques}[1]{{\color{blue}#1?}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{\uline{#1}}}}
\ignore{
    \newcommand{\jnote}[1]{% using fixme
    	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
    	\renewcommand{\fixmelogo}{}%
    	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
                {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
                \textit{\color{mydarkgreen}#1}}}}%
    }
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END newcommands for ignoring, commenting, ....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> newcommands-labels-refs.tex <==
% label and ref newcommands
% now mostly deprecated (but redefined and kept for backward compatibility) - move to \cref from the cleveref package
\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\Crefname{equation}{}{}

%DONE: xyzref{} should be able to handle multiple arguments so that you can
%reference multiple figures/equations at the same time -AG
%Now fixed with some package/command CREF.
\newcommand{\corrlabel}[1]{\label{corr:#1}}
\newcommand{\corrref}[1]{Corollary \ref{corr:#1}}
\newcommand{\assref}[1]{Assumption \ref{ass:#1}}
\newcommand{\asslabel}[1]{\label{ass:#1}}
%\newcommand{\eqnref}[1]{(\ref{eq:#1})}
%\newcommand{\eqnlabel}[1]{\label{eq:#1}}
\newcommand{\eqnlabel}[1]{\label{#1}}
\newcommand{\eqnref}[1]{\cref{#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figlabel}[1]{\label{#1}}
\newcommand{\figref}[1]{\cref{#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\exampleref}[1]{Example~\ref{ex:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\thlabel}[1]{\label{th:#1}}
\newcommand{\thref}[1]{Theorem~\ref{th:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem \ref{thm:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma \ref{lem:#1}}
\newcommand{\examplelabel}[1]{\label{ex:#1}}
\newcommand{\labexample}[1]{\label{example:#1}}
\newcommand{\refexample}[1]{Example{ }\ref{example:#1}}
\newcommand{\httpref}[1]{}
\let\el=\eqnlabel
\let\er=\eqnref


==> newcommands-math.tex <==
\newcommand{\ddt}[2]{{\frac{d}{d #2}\left. #1 \right.}}
\newcommand{\ddx}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\Ddx}[2]{{\frac{D}{d{#2}}\left[ #1 \right]}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\deq}{=}
\newcommand{\I}{I\left[\right]}
\newcommand{\ELL}[1]{L\left[#1\right]}
\newcommand{\w}{\omega}
\newcommand{\calD}{{\cal D}}
\renewcommand{\jmath}{j}
\newcommand{\Pinvt}{{P(t)}^{-1}}
\newcommand{\halmos}{\hskip\textwidth minus\textwidth \rule{6pt}{6pt}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calAT}{{\cal A}^T}
\newcommand{\calL}{{\cal L}}
\newcommand{\calLadj}{\calL^\dagger}
\newcommand{\calR}{{\cal R}}
\newcommand{\Reals}{\Bbb{R}}
\newcommand{\Real}{\Bbb{R}}
\newcommand{\Safe}{\ensuremath{{\bf S}}}
\newcommand{\Pade}{{Pad\'e}}
\newcommand{\Complexes}{\Bbb{C}}
\newcommand{\HvecqLanc}{\Hvec^{(L)}_q}
\newcommand{\HvecqArn}{\Hvec^{(A)}_q}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\calDT}{{\cal D}^T}
\newcommand{\calCtil}{\tilde{\cal C}}
\newcommand{\calJtil}{\tilde{\cal J}}
\newcommand{\calDtil}{\tilde{\cal D}}
\newcommand{\JstarDphi}{J_{\Delta \phi}^*}
\newcommand{\Jstarphi}{J_{\phi}^*}
\newcommand{\vecbphi}{\vec b_{\phi}}
\newcommand{\vecbext}{\vec b_{\text{ext}}}
\newcommand{\phistarIdeal}{\phi_{\text{ideal}}^*}
\newcommand{\apdx}[1]{\appref{#1}} 
\newcommand{\delbydel}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\delbydeln}[3]{\ensuremath{\frac{\partial^{{#1}}
{#2}}{\partial{#3}^{{#1}}}}}
\newcommand{\delbydelat}[3]{\ensuremath{\left. \frac{\partial
{#1}}{\partial {#2}} \right|_{{#3}}}}
\newcommand{\dee}{\ensuremath{\mathrm{d}}}
\newcommand{\dbyd}[2]{\ensuremath{\frac{\mathrm{d} {#1}}{\mathrm{d}
{#2}}}}
\newcommand{\dbydn}[3]{\ensuremath{\frac{\mathrm{d}^{{#1}}{#2}}
{\mathrm{d}{#3}^{{#1}}}}}
\newcommand {\dist}[1] {{{\rm dist}\left({#1}\right)}}
\def\Matrix#1{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\textdiag}{{\text{diag}}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\del}{\nabla}
\newcommand{\Rxx}{R_{\vec x \vec x}}
\newcommand{\Sxx}{S_{\vec x \vec x}}
\newcommand{\Snn}{S_{\vec n \vec n}}
\newcommand{\vecphi}{\vec \phi}
\newcommand{\Dphi}{\Delta \phi}
\newcommand{\vecDphi}{\vv{\Delta \phi}}
\newcommand{\dphi}{\delta \phi}
\newcommand{\vecdphi}{\vv{\delta \phi}}
\newcommand{\ah}{\alpha_g} % g for group
%\newcommand{\tDagger}{{\tilde t}}
\newcommand{\tDagger}{{t^{\!\dagger}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\texthyphen}{\text{--}}

%The substack command can be used to produce a multi-line subscripts or superscripts:
%\sum_{\substack{0\le i\le m\\ 0<j<n}} P(i,j) produces a two-line subscript underneath the sum.
%A slightly more general form is the subarray environment which allows you to specify that each line should be left-aligned instead of centered, as here:
% \sum_{\begin{subarray}{l} i\in\Lambda\\ 0<j<n \end{subarray}} P(i,j) 

%\newcommand{\be}[1]{\begin{equation}\eqnlabel{#1}} % now moved to cleveref
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\def\ee{\end{equation}}


==> newcommands-squeeze-spaces.tex <==
%%% tweaklist renewcommands
\newcommand{\modifiedListParamters}{
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.1em}
  \setlength{\partopsep}{0em}
  \setlength{\parsep}{0em}
  \setlength{\leftmargin}{1.1em}
  \setlength{\itemindent}{0.0em}
}
\renewcommand{\enumhook}{
  \modifiedListParamters
  \setlength{\itemindent}{0.2em}
}
\renewcommand{\itemhook}{
  \modifiedListParamters
}
\renewcommand{\descripthook}{
  \modifiedListParamters
  \setlength{\itemindent}{-1.0em}
}
%%% end tweaklist renewcommands

\ignore{not usually needed, but the definitions have useful info
		Space saving List environment for enumerations.

	\newcounter{myctr}
	\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
   		{\usecounter{myctr}
   		%\setlength{\topsep}{1mm}\setlength{\itemsep}{0.5mm}
   		\setlength{\topsep}{0.3mm}
   		\setlength{\itemsep}{0mm}
   		\setlength{\parsep}{0.3mm}
   		\setlength{\itemindent}{0mm}
   		\setlength{\partopsep}{0mm}
   		\setlength{\labelwidth}{15mm}
   		\setlength{\leftmargin}{4mm}
   		}
	}{\end{list}}

	\newenvironment{myitemize}{\begin{list}{$\bullet$}
	  \ignore{\setlength{\topsep}{0.8mm}\setlength{\itemsep}{0.25mm}}
	  {\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
	  \setlength{\parsep}{0.1mm}
	  \setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
	  \setlength{\labelwidth}{15mm}
	  \setlength{\leftmargin}{4mm}}
	}{\end{list}}
}

%%%% titlesec: squeezing whitespace between section headings
	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
                                           % space above; {*0.5} is space below
	\titlespacing{\subsection}{0pt}{*0.1}{*0}
	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%% end titlesec

%%%% squeezing whitespace in and around figures
    \floatsep=0em % space left between floats.
    \textfloatsep=0em % space between last top float or first bottom float and the text.
    \intextsep=0em % space left on top and bottom of an in-text float.
    %\dbltextfloatsep is \textfloatsep for 2 column output.
    %\dblfloatsep is \floatsep for 2 column output.
    \abovecaptionskip=0em % space above caption
    \belowcaptionskip=0em % space below caption
%%%% END squeezing whitespace in and around figures

\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

%\newcommand{\mycaption}[1]{\caption{\small #1}}
\newcommand{\mycaption}[1]{\caption{\tiny #1}}

% for captions spacing
\captionsetup[table]{font={scriptsize},format=hang,indention=0em}     %% change 1.2 as you like
\captionsetup[figure]{font={scriptsize},format=hang,indention=0em}    %% change as you like
 %% or
 %% \captionsetup{font={stretch=1.2}}  %% this affects both figure and table

% replace Figure x in captions by Fig. x
%\renewcommand{\figurename}{Fig.} % doesn't work.
%but \usepackage[figurename=Fig.]{caption} in packages-headers.tex does work.


%\renewcommand{\baselinestretch}{1.5}
%\setstretch{1.5}

%\def\baselinestretch{0.8593}\large\normalsize - this form works locally?
%\renewcommand{\baselinestretch}{0.94} - this form works only in the preamble
%\renewcommand{\baselinestretch}{0.90}
%\renewcommand{\baselinestretch}{0.5}
%\linespread{0.5} % 0.5 -> 7 lines per inch; 0.9 -> a bit more than 6 lines 
%                 % per vertical inch
% \linespread{0.99}

% baselinestretch fixes for squeezing. See also linespread
%\def\ssp{\def\baselinestretch{0.95645}\large\normalsize} % "single space"
%\def\ssp{\def\baselinestretch{0.905}\large\normalsize} % "single space"
\def\ssp{\def\baselinestretch{0.9}\large\normalsize} % "single space"
\def\dsp{\def\baselinestretch{1.35}\large\normalsize} % "double space"
\ssp

% indent paragraphs less (saves space)
\parindent 	1em
% do not indent paragraphs (saves more space)
\parindent 	0em
% adjust space between paragraphs (0em can obscure paragraph breaks)
\parskip 0.3em


==> newcommands-thm-env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EndProof{\hfill \quad \vrule width 1ex height 1ex depth 0pt  }
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{illustration}{Illustration}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newenvironment{sketch}{\noindent{\bf Sketch of Proof}:}{\halmos}
\newenvironment{conjecture}{\noindent{\bf Conjecture}: \em}{}
\newcommand{\numberedtheorem}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thetheorem
		\renewcommand{\thetheorem}{#1}
	}
	\begin{theorem}
	\ifthen{\not\equal{#2}{}}{
		\thmlabel{#2}
	}
	#3
	\end{theorem}
	\ifthen{\not\equal{#1}{}}{
		\let\thetheorem=\oof
		\addtocounter{theorem}{-1}
	}
}
\newcommand{\numberedlemma}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thelemma
		\renewcommand{\thelemma}{#1}
	}
	\begin{lemma}
	\ifthen{\not\equal{#2}{}}{
		\lemlabel{#2}
	}
	#3
	\end{lemma}
	\ifthen{\not\equal{#1}{}}{
		\let\thelemma=\oof
		\addtocounter{lemma}{-1}
	}
}


==> packages-headers.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
%\RequirePackage[usenames]{pstcol} 
\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsthm,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage{hyperref} 
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{MyDarkRed}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}


\input newcommands-colours
\input newcommands-highlight-ignore
\input newcommands-eg-ie-etc
\input newcommands-labels-refs
\input newcommands-math
\input newcommands-thm-env
\input newcommands-for-bibtex
\input newcommands-squeeze-spaces


==> response.tex <==
\clearpage
\section*{\normalfont {\large Response to Reviewers' Comments}}

{\it
The reviewers have raised a number of serious questions. Mainly, they are about
(a) Utility of this definition compared to looking at amplitude decay after
introducing a disturbance, (b) Possible ambiguity in the definition in more
complicated oscillators, (c) Some inconsistencies in the numerical examples,
and (d) Ways to calculate this in practice. Please revise the manuscript
responding to all of the reviewers' queries.  Perhaps some of the examples can
be shortened to make room for more rigorous explanations.
}
\vspace{1em}

(a) and (b) are actually related to the same issue with the previous version of
this paper.
The observation of amplitude decay provides us with the intuition behind the
definition of \Q{} factor; while the more rigorous LPTV-based formulation is
the actual definition, and it is generalizable to more complicated oscillators.
In the revision, we have modified the introduction, changed Section II's title
and added more discussion to Section III to make this point clear.
We have also fixed inconsistencies with the numerical results.

As for (d), the step-by-step description of the algorithm is provided in
Section IV.
We have added more details about our implementations. And we plan to release
our implementations as open-source software under the GNU General Public
License.
Admittedly, the proposed numerical characterization routine is not yet
available in commercial simulators; this is a new concept and algorithm after
all.
But as we mentioned in Section IV, ``there are well-developed numerical
techniques for each step in the calculation of \Q{}'', ``many implementations
are already available today in open-source and commercial simulators for
oscillator phase noise analysis''.
In fact, anonymous reviewer 3 appears to be able to implement the algorithm
based on the paper during the review process.
If the paper is published, it is probably not too unreasonable to expect that
even implementations in commercial simulations will become available.

Moreover, the example section has been shortened.

In the revision, we also added in citation a very recent {\it Science} paper
({\it Tsakmakidis 2017})
% \cite{tsakmakidis2017QfactorScience}
that discusses the \Q{} factor of linear
resonators from physicists' perspective.
Specifically, it shows that energy dissipation and bandwidth of a linear system
can be decoupled.
It appears that researchers have just started to question the validity of using
a single \Q{} factor for characterizing linear resonators.
The comparison of the several \Q{} factor definitions for nonlinear
oscillators, including the new one we propose, may be a timely contribution
from the circuit community on a similar subject.


\vspace{2em}
{\it
Reviewers' Comments to the Authors:

Reviewer: 1

Comments to the Author

In this paper, the authors provide a definition of the quality factor of
oscillators which can be applied to any topology and even to non-electrical
oscillators.

Although the proposed formulation of Q factor is interesting, however, in my
opinion, the advance of theory provided by the paper is quite limited and so is
the utility for circuit designers. I suggest to resubmit a shortened version of
the paper to TCAS-II.

More in detail:

1) In the end, the computation of the second eigenvalue of the state-transition
matrix (and, hence, the Q factor) needs circuit simulations. Therefore, the
proposed method offers only little or no improvement with respect to an
estimation of Q based on the observation of amplitude settling time using
transient simulations.
}
\vspace{1em}

Observation of amplitude settling behaviour is where we derive the intuition
behind this \Q{} factor formulation; it is not a replacement for the LPTV
formulation. The paper has been modified (in introduction, section title, and
additional discussions in Section III) to make this point clearer.

Besides, defining \Q{} for nonlinear oscillators based on amplitude decay is
new in itself.
The LPTV formulation and numerical calculation are there to consolidate this
intuition.

\vspace{1em}
{\it
2) Authors do not take into account the possibility of a third eigenvalue very
close (in magnitude) to the second. In such a situation, the definition of Q
proposed by the authors becomes not so meaningful. Therefore, I suspect that
the proposed theory lacks of generality. Authors should comment about that.
}
\vspace{1em}

LPTV systems are in a way just like regular linear systems --- there is
superposition of responses generated by different multipliers, and normally
only the slowest multiplier is considered (except for the multiplier equal to
1, which represents the unstable phase of oscillation).
Indeed, when other multipliers are close to the slowest one, the response can
be more complicated than a simple exponential decay.
This is a limitation of the proposed Q factor, and we commonly encounter such
limitation whenever we try to use a scalar figure of merit for characterizing
systems, even regular linear systems.
We have revised the paper to comment on this limitation.

\vspace{1em}
{\it
3) In Section V, authors should give a better proof of validity of the proposed
method of calculation of Q. In particular, they should show that the speed of
the amplitude settling numerically matches with the simulated lambda2.
}
\vspace{1em}

In Section V-B, we have actually simulated the transient amplitude decay. In
the revision, we added discussions on the comparison between amplitude decay
observation and LPTV-based formulation.

We have also revised the paper to make it clear that the amplitude decay is
where the intuition comes from. It need not numerically match the LPTV-based
formulation exactly. In fact, amplitude settling is not easy to simulate
properly. Perturbation has to be small, otherwise it does not reflect the
oscillator's quality close to the limit cycle. Then 5\% of that becomes even
smaller, making it hard to observe in the presence of numerical errors and
tolerances.
Also, precisely as the reviewers pointed out, the direction of the perturbation
matters. That's why the LPTV-based formulation is a better, more elegant
solution to defining \Q{} more rigorously.

\vspace{1em}
{\it
4) Authors should explain how it is possible to extract the value of lambda2 in
commercial simulators such as SpectreRF (if that is possible, of course).
Otherwise, I suspect that the proposed definition is not really useful in
practical circuit design.
}
\vspace{1em}

The proposed algorithm is described step by step in the manuscript for
reproducibility. We plan to also release our implementations under GPL.
As a new algorithm, the numerical routine for calculating the proposed \Q{} is
not yet built-in in SpectreRF.
But unlike most new simulation algorithms, it does not require structural
change to existing infrastructure; for people who have access to the internals
of commercial simulators, it is not difficult to implement. 
So chances are higher for it to be adopted by commercial simulators.


\vspace{1em}
{\it
Reviewer: 2

Comments to the Author In this paper the author discuss the extension of the
quality factor concept to nonlinear oscillators. The paper is interesting, it
is well written and well organized, but in my personal opinion is not suitable
for publication.

First problem is that the Q factor introduced in the paper is ill defined. The
authors define the Q factor as the ration between an extra energy applied to
the system and an extra energy dissipated. I expect that the ratio depend on
both how much extra energy is applied, and on how it is applied.

The authors are aware of this and they suggest as a solution that the ratio
should converge by taking some limit. No prove of convergence is given, neither
are given arguments to justify the convergence. It is not explained what kind
of limit should be considered. It seems to me that asymptotically, as the
trajectory approaches the limit cycle, the extra energy dissipated per cycle
will become zero, and according to the proposed definition the Q factor should
become infinite for every stable nonlinear oscillator.
}
\vspace{1em}

This is actually not true, since \Q{} represents the ratio between the extra
energy and the dissipated energy. If both go to zero, it is hard to take the
limit by observing the transient waveforms. That's part of the reason why we
define \Q{} more rigorously using LPTV theory. A LPTV system is a special type
of linear system; its behaviour does not depend on the size of the perturbation.
Its slowest moment, characterized by $\lambda_2$, is what we use to define \Q{}
factor.

In the revision, we have modified the flow of the paper to underscore the
limitations in directly applying the physical intuition for \Q{}
characterization, and added discussion on how the LPTV-based formulation is
related to the intuition. Exactly as the reviewers pointed out, how the energy
is applied matters.
In Section III, we show that the slowest moment is the one along the direction
of the eigenvector associated with $\lambda_2$ (the one associated with
$\lambda_1$ is the PPV), which will dominate in the settling behaviour.

\vspace{1em}
{\it
In section III the authors use Floquet theory to derive a formula for the Q
factor. Q is defined as the natural logarithm of the (modulus of) second
largest Floquet multiplier, eq (16). I have two concerns. First: this formula
looks marginally related to the previous energy based definition. No energy
considerations are made in the derivation. In particular, energy "spreads"
along all directions, why considering only one component? What if there are two
or more Floquet's multipliers with the same modulus?
}
\vspace{1em}

We have added discussion of the relationship between the energy-based intuition
and the LPTV-based formulation in the revision. In short, the Floquet
multipliers characterize the settling behaviour of the amplitude, not energy.
The concept of ``energy'' is specific to certain circuit topologies, and cannot
be inferred just from oscillator equations. In fact, for some oscillators such
as spin-torque and chemical reaction oscillators, it is hard to pinpoint where
the energy is. However, we normally assume energy $E$ to be proportional to the
amplitude of the limit cycle, which makes $\Delta E$ proportional to the change
of amplitude. So we can say $\Delta E$ is dissipated in the same rate as the
decaying amplitude. Thus the LPTV-based formulation is related to, but more
rigorous and general than the energy-based intuition.

Reviewer 1 asked a similar question about the choice of $\lambda_2$; we would
like to refer you to our responses there. To fully analyze the oscillator,
we will need the whole spectrum of multipliers.
But to characterize the oscillator using only a scalar figure of merit, which
we often want in engineering, it is not unreasonable to choose the slowest
component governed by $\lambda_2$. We have commented on this limitation of
scalar figures of merit in the revision.

\vspace{1em}
{\it
Second: Q gives the same information provided by lambda\_2, and we need to
compute lambda\_2 in order to calculate Q. Then why should we care of Q?
It is a trivial application of Occam's razor, I see no advantage in considering
this Q factor. It does not introduce anything new.
}
\vspace{1em}

\Q{} factor is a commonly used concept in engineering, while $\lambda_2$ is a
term more mathematically oriented. In this case, \Q{} has a energy-based
physical intuition behind it, making it more suitable to use.
% Why do we ever use any scalar figure of merit then when we have all the circuit
% equations available? 

\vspace{1em}
{\it
Minor: on page 2 the authors write: "The higher the Q factor, the more slowly
its amplitude responds to perturbations, and the more stable the limit cycle".
I am puzzled. In a strongly stable system, amplitude response is almost
immediate, e.g. amplitude perturbations are quickly damped. Since Q is
proportional to ln|lamba\_2|, the higher the Q factor, the smaller |lambda\_2|,
the more stable the system (the faster amplitude perturbations are damped).
}
\vspace{1em}

This is an excellent point!
Our \Q{} definition is analogous to that for linear resonators --- a higher
value means slower settling.
The strongly stable system mentioned above is actually a very lossy system.
So in some applications, you may want this \Q{} factor to be low.
We have to admit that a definition of \Q{} that captures all the ``good
qualities'' of oscillators is a common myth in engineering. As discussed in
Section VI, our formulation is an addition to the existing ones; we point out
an counterintuitive and often overlooked fact that there is no equivalence
between them for nonlinear oscillators.

\vspace{1em}
{\it
Reviewer: 3

Comments to the Author

My overall opinion about the paper is that it is interesting and well written,
but in some way too long, with an excess of numerical examples and with some
considerations that are repeated several times. I suggest to shorted it. The
examples are taken from different areas but from my standpoint the key aspect
is the structure of the DAE they generate. Same DAE formulations and
characteristics mean same properties. The key aspect of the paper is the
determination of the second largest Floquet multiplier in a stable oscillator.
I tried to repeat one your numerical evaluation of the reported values and my
result does not match yours. I did this with the LC-oscillator. Please could
you check values ? It seems to me that the explanation after Fig. 3. on  how
the value of $\lambda_2$ is related to the large/small Q is wrong. There are
"swaps" among "low-Q" and "high-Q". Furthermore the other examples can not be
replicated. I tried with the BJT phase-shift oscillator but the characteristic
of the BJT is unknown.
}
\vspace{1em}

We have shortened the examples and removed some repetitions in the paper.
Although in Section VI, we repeated some definitions and considerations. And we
hope to keep them, so that the contents are more useful in clarifying concepts
in the field.

Yes, our formulation works on oscillators' DAEs, as opposed to certain
topologies. For a reviewer who is an expert in the field, we need not say more.
But for general audience, we need to show at least one non-electrical example,
such as the STNO. The chemical reaction example serves a different purpose
since it is not an amplitude-stable oscillator. Such conservative systems are not
often seen in electrical circuits, which are normally dissipative. So we hope
to keep that. The BJT phase-shift oscillator example is removed, since it does
not offer much new.

There were actually some inconsistencies with the values for LC oscillators; we
have now fixed them. The BJT example, although removed in the revision, used
Ebers-Moll model with $\alpha_F=0.99$, $\alpha_R=0.5$ and $I_S = 10^{-12}A$,
$V_T = 0.025V$ for the diodes inside, without capacitance model. You may check
the results if you would like to.

\vspace{1em}
{\it
In a complex circuit there can be several state variables. In this case second
largest Floquet multiplier is not necessarily related to the oscillator
subcircuit. A trivial example is a simple RC circuit (in a limit case a
floating capacitor) that introduces a Floquet multiplier (almost) equal to
(almost). Any comment ?
}
\vspace{1em}

If the circuit of interest is an oscillator, we would say that everything in it
counts. In the extreme case, if there is a floating capacitor in the
oscillator, then it is not amplitude stable since it may never recover from
perturbations.
I suppose the problem is not with the complexity of the oscillator, but with
the question whether the circuit is an oscillator.
But how to detect it is a very valid question; it requires combining PSS
responses and eigenanalysis of monodromy matrix in an intelligent way. And we
have added it as part of future work of this paper.

